Quantifying the Information Leak in Cache Attacks through Symbolic Execution

Cache timing attacks allow attackers to infer the properties of a secret execution by observing cache hits and misses. But how much information can actually leak through such attacks? For a given program, a cache model, and an input, our CHALICE framework leverages symbolic execution to compute the amount of information that can possibly leak through cache attacks. At the core of CHALICE is a novel approach to quantify information leak that can highlight critical cache side-channel leaks on arbitrary binary code. In our evaluation on real-world programs from OpenSSL and Linux GDK libraries, CHALICE effectively quantifies information leaks: For an AES-128 implementation on Linux, for instance, CHALICE finds that a cache attack can leak as much as 127 out of 128 bits of the encryption key.

==> results/plots/AES/plot_script_test_compare <==
set terminal postscript color
set output 'aes_byte_leak_count_compare.eps'
#set size 1.2,1.0
#set grid
set title "Cache side-channel leak in AES (observation via miss count)"
set ylabel "#values leaked per byte"
set xlabel "Key bytes"
#set xrange [1:16]
#set yrange [1:55]
#set logscale y
#set xtics ("" 0, "cnt" 1, "fir" 2, "fdct" 3, "expint" 4, "qurt" 5, "nsichneu" 6, "edn" 7, "ludcmp" 8, "ns" 9, "ndes" 10, "bsort100" 11, "adpcm" 12, "st" 13)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3, "5" 4, "6" 5, "7" 6, "8" 7, "9" 8, "10" 9, "11" 10, "12" 11, "13" 12, "14" 13, "15" 14, "16" 15)
#set xtics mirror rotate by -45
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
#set style data linespoints

plot 'aes_byte_leak_count_compare.dat' using 1 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 2 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 8KB, 2-way (observation via miss count)"
set output 'aes_byte_leak_count_compare_1.eps'

plot 'aes_byte_leak_count_compare.dat' using 3 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 4 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 8KB, 4-way (observation via miss count)"
set output 'aes_byte_leak_count_compare_2.eps'

plot 'aes_byte_leak_count_compare.dat' using 5 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 6 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 16KB, 2-way (observation via miss count)"
set output 'aes_byte_leak_count_compare_3.eps'

plot 'aes_byte_leak_count_compare.dat' using 7 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 8 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 16KB, 4-way (observation via miss count)"
set output 'aes_byte_leak_count_compare_4.eps'

plot 'aes_byte_leak_count_compare.dat' using 9 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 10 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 32KB, 2-way (observation via miss count)"
set output 'aes_byte_leak_count_compare_5.eps'

plot 'aes_byte_leak_count_compare.dat' using 11 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 12 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 32KB, 4-way (observation via miss count)"
set output 'aes_byte_leak_count_compare_6.eps'

plot 'aes_byte_leak_count_compare.dat' using 13 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 14 fs solid 1.0 lt -1 title 'AES from OpenSSL'


set title "Cache side-channel leak in AES (observation via hit/miss sequence length 1)"
set output 'aes_byte_leak_seq_compare.eps'

plot 'aes_byte_leak_seq_compare.dat' using 1 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 3 fs solid 1.0 lt -1 title 'AES from OpenSSL'


==> results/plots/AES/plot_script_test_count_sens_per_byte <==
set terminal postscript color
set output 'aes_basic_byte_leak_count_sens.eps'
#set size 1.2,1.0
#set grid
set title "Cache side-channel leak in AES (basic crypto) w.r.t. cache configurations (observation via miss count)"
set ylabel "#values leaked per byte" 
set xlabel "Key bytes"
#set xrange [1:10]
set yrange [1:220]
#set logscale y
#set xtics ("2-way, 8KB" 0, "4-way, 8KB" 1, "2-way, 16 KB" 2, "4-way, 16KB" 3, "2-way, 32 KB" 4, "4-way, 32 KB" 5)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3, "5" 4, "6" 5, "7" 6, "8" 7, "9" 8, "10" 9, "11" 10, "12" 11, "13" 12, "14" 13, "15" 14, "16" 15)
#set xtics mirror rotate by 45
#rotate parallel
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
#set style data linespoints

plot 'aes_byte_leak_sensitivity_count.dat' using 1 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 2 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 3 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 4 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 5 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 6 fs pattern 4.66 lt -1 title '4-way, 32 KB'


set title "Cache side-channel leak in AES (OpenSSL) w.r.t. cache configurations (observation via miss count)"
set output 'aes_openssl_byte_leak_count_sens.eps'
set yrange [1:25]

plot 'aes_byte_leak_sensitivity_count.dat' using 13 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 14 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 15 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 16 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 17 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 18 fs pattern 4.66 lt -1 title '4-way, 32 KB'


==> results/plots/AES/plot_script_test_seq_sens_per_byte <==
set terminal postscript color
set output 'aes_basic_byte_leak_seq_sens.eps'
#set size 1.2,1.0
#set grid
set title "Information leak in AES (basic crypto) w.r.t. cache configurations (observation via hit/miss sequence length 1)"
set ylabel "#values leaked per byte" 
set xlabel "Key bytes"
#set xrange [1:10]
set yrange [1:256]
#set logscale y
#set xtics ("2-way, 8KB" 0, "4-way, 8KB" 1, "2-way, 16 KB" 2, "4-way, 16KB" 3, "2-way, 32 KB" 4, "4-way, 32 KB" 5)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3, "5" 4, "6" 5, "7" 6, "8" 7, "9" 8, "10" 9, "11" 10, "12" 11, "13" 12, "14" 13, "15" 14, "16" 15)
#set xtics mirror rotate by 45
#rotate parallel
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
#set style data linespoints

plot 'aes_byte_leak_sensitivity_seq.dat' using 1 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 2 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 3 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 4 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 5 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 6 fs pattern 4.66 lt -1 title '4-way, 32 KB'


set output 'aes_openssl_byte_leak_seq_sens.eps'
#set yrange [1:]
set title "Information leak in AES (OpenSSL) w.r.t. cache configurations (observation via hit/miss sequence length 1)"

plot 'aes_byte_leak_sensitivity_seq.dat' using 13 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 14 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 15 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 16 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 17 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 18 fs pattern 4.66 lt -1 title '4-way, 32 KB'


==> results/plots/AES/seq_access_key_bound_script <==
#!/bin/bash

grep -inr "\[++\]" $1 > scripts/leak
while read line; do
	access=$(echo $line | cut -f10 -d" ")
	byte=$(echo $line | cut -f8 -d" ")
	echo $access
	byte=$(echo $byte | rev | cut -c 2- | rev)
	echo $byte
	echo $line >> temp/record_byte_leak_from_hit_sequence_${access}_${byte}
done <scripts/leak
grep -inr "\[--\]" $1 > scripts/leak
while read line; do
	access=$(echo $line | cut -f10 -d" ")
	byte=$(echo $line | cut -f8 -d" ")
	echo $access
	byte=$(echo $byte | rev | cut -c 2- | rev)
	echo $byte
	echo $line >> temp/record_byte_leak_from_miss_sequence_${access}_${byte}
done <scripts/leak



==> results/plots/AES/splot_script_test <==
# set terminal svg size 600,400 dynamic enhanced fname 'arial'  fsize 10 mousing name "surface1_1" butt dashlength 1.0 
# set output 'surface1.1.svg'
set grid nopolar
set grid xtics nomxtics ytics nomytics noztics nomztics \
 nox2tics nomx2tics noy2tics nomy2tics nocbtics nomcbtics
set grid layerdefault   lt black linewidth 0.200,  lt black linewidth 0.200
set hidden3d back offset 1 trianglepattern 3 undefined 1 altdiagonal bentover
set style data lines
set title "3D surface from a grid (matrix) of Z values" 
set xrange [ -0.500000 : 4.50000 ] noreverse nowriteback
set yrange [ -0.500000 : 4.50000 ] noreverse nowriteback
x = 0.0
splot plots/aes_byte_leak_count.dat with lines notitle



==> results/plots/DES/plot_script_test_compare <==
set terminal postscript color
set output 'des_byte_leak_count.eps'
#set size 1.2,1.0
#set grid
set title "Cache side-channel leak in OpenSSL DES (observation via miss count)"
set ylabel "#values leaked per byte"
set xlabel "Key bytes"
#set xrange [1:16]
#set yrange [1:55]
#set logscale y
#set xtics ("" 0, "cnt" 1, "fir" 2, "fdct" 3, "expint" 4, "qurt" 5, "nsichneu" 6, "edn" 7, "ludcmp" 8, "ns" 9, "ndes" 10, "bsort100" 11, "adpcm" 12, "st" 13)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3, "5" 4, "6" 5, "7" 6, "8" 7)
#set xtics mirror rotate by -45
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
#set style data linespoints

plot 'des_count.dat' using 1 fs solid 0.11 lt -1 title '1-way, 4KB',\
			'' using 2 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 3 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 4 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 5 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 6 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 7 fs pattern 4.66 lt -1 title '4-way, 32 KB'


set output 'des_byte_leak_seq.eps'
set title "Cache side-channel leak in OpenSSL DES (observation via hit/miss sequence length 1)"

plot 'des_seq.dat' using 1 fs solid 0.11 lt -1 title '1-way, 4KB',\
			'' using 2 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 3 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 4 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 5 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 6 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 7 fs pattern 4.66 lt -1 title '4-way, 32 KB'



==> results/plots/GDK/plot_script_test_count_sens_per_byte <==
set terminal postscript color
set output 'gdk_byte_leak_count_sens.eps'
#set size 1.2,1.0
set title "Average cache side-channel leak in GDK routines w.r.t. cache configurations (observation via miss count)"
set ylabel "#values leaked per byte"
set xlabel "Input bytes"
#set xrange [1:10]
set yrange [1:260]
#set logscale y
#set xtics ("2-way, 8KB" 0, "4-way, 8KB" 1, "2-way, 16 KB" 2, "4-way, 16KB" 3, "2-way, 32 KB" 4, "4-way, 32 KB" 5)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3)
#set xtics mirror rotate by 45
#rotate parallel
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above

plot 'gdk_byte_leak.dat'  using 1 fs solid 0.11 lt -1 title '1-way, 8KB',\
			'' using 2 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 3 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 4 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 5 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 6 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 7 fs pattern 4.66 lt -1 title '4-way, 32 KB'



==> results/plots/GDK/plot_script_test_seq_sens_per_byte <==
set terminal postscript color
set output 'gdk_byte_leak_seq_sens.eps'
#set size 1.2,1.0
set title "Average cache side-channel leak in GDK routines w.r.t. cache configurations (observation via miss sequence)"
set ylabel "#values leaked per byte"
set xlabel "Input bytes"
#set xrange [1:10]
set yrange [1:260]
#set logscale y
#set xtics ("2-way, 8KB" 0, "4-way, 8KB" 1, "2-way, 16 KB" 2, "4-way, 16KB" 3, "2-way, 32 KB" 4, "4-way, 32 KB" 5)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3)
#set xtics mirror rotate by 45
#rotate parallel
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above

plot 'gdk_byte_leak_seq.dat'  using 1 fs solid 0.11 lt -1 title '1-way, 8KB',\
			'' using 2 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 3 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 4 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 5 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 6 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 7 fs pattern 4.66 lt -1 title '4-way, 32 KB'



==> results/plots/RC4/plot_script_test_compare <==
set terminal postscript color
set output 'rc4_byte_leak_count.eps'
#set size 1.2,1.0
#set grid
set title "Cache side-channel leak in OpenSSL RC4 (observation via miss count)"
set ylabel "#values leaked per byte"
set xlabel "Key bytes"
#set xrange [1:16]
#set yrange [1:55]
#set logscale y
#set xtics ("" 0, "cnt" 1, "fir" 2, "fdct" 3, "expint" 4, "qurt" 5, "nsichneu" 6, "edn" 7, "ludcmp" 8, "ns" 9, "ndes" 10, "bsort100" 11, "adpcm" 12, "st" 13)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3, "5" 4, "6" 5, "7" 6, "8" 7)
#set xtics mirror rotate by -45
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
#set style data linespoints

plot 'rc4_count.dat' using 1 fs solid 0.11 lt -1 title '1-way, 4KB',\
			'' using 2 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 3 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 4 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 5 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 6 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 7 fs pattern 4.66 lt -1 title '4-way, 32 KB'


set output 'rc4_byte_leak_seq.eps'
set title "Cache side-channel leak in OpenSSL RC4 (observation via hit/miss sequence length 1)"

plot 'rc4_seq.dat' using 1 fs solid 0.11 lt -1 title '1-way, 4KB',\
			'' using 2 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 3 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 4 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 5 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 6 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 7 fs pattern 4.66 lt -1 title '4-way, 32 KB'



==> results/scripts/plot_script_test_compare <==
set terminal postscript color
set output 'plots/aes_byte_leak_count_compare.eps'
#set size 1.2,1.0
#set grid
set title "Cache side-channel leak in AES (observation via miss count)"
set ylabel "No. of impossible values/byte (inforrmation leak)"
set xlabel "Key bytes"
#set xrange [1:16]
#set yrange [1:55]
#set logscale y
#set xtics ("" 0, "cnt" 1, "fir" 2, "fdct" 3, "expint" 4, "qurt" 5, "nsichneu" 6, "edn" 7, "ludcmp" 8, "ns" 9, "ndes" 10, "bsort100" 11, "adpcm" 12, "st" 13)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3, "5" 4, "6" 5, "7" 6, "8" 7, "9" 8, "10" 9, "11" 10, "12" 11, "13" 12, "14" 13, "15" 14, "16" 15)
#set xtics mirror rotate by -45
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
#set style data linespoints

plot 'plots/aes_byte_leak_count_compare.dat' using 1 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 2 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 8KB, 2-way (observation via miss count)"
set output 'plots/aes_byte_leak_count_compare_1.eps'

plot 'plots/aes_byte_leak_count_compare.dat' using 3 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 4 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 8KB, 4-way (observation via miss count)"
set output 'plots/aes_byte_leak_count_compare_2.eps'

plot 'plots/aes_byte_leak_count_compare.dat' using 5 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 6 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 16KB, 2-way (observation via miss count)"
set output 'plots/aes_byte_leak_count_compare_3.eps'

plot 'plots/aes_byte_leak_count_compare.dat' using 7 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 8 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 16KB, 4-way (observation via miss count)"
set output 'plots/aes_byte_leak_count_compare_4.eps'

plot 'plots/aes_byte_leak_count_compare.dat' using 9 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 10 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 32KB, 2-way (observation via miss count)"
set output 'plots/aes_byte_leak_count_compare_5.eps'

plot 'plots/aes_byte_leak_count_compare.dat' using 11 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 12 fs solid 1.0 lt -1 title 'AES from OpenSSL'

set title "Cache side-channel leak in AES, cache = 32KB, 4-way (observation via miss count)"
set output 'plots/aes_byte_leak_count_compare_6.eps'

plot 'plots/aes_byte_leak_count_compare.dat' using 13 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 14 fs solid 1.0 lt -1 title 'AES from OpenSSL'


set title "Cache side-channel leak in AES (observation via hit/miss sequence length 1)"
set output 'plots/aes_byte_leak_seq_compare.eps'

plot 'plots/aes_byte_leak_seq_compare.dat' using 1 fs pattern 1.33 lt -1 title 'AES from basic Crypto',\
		 '' using 3 fs solid 1.0 lt -1 title 'AES from OpenSSL'


==> results/scripts/plot_script_test_count_sens_per_byte <==
set terminal postscript color
set output 'plots/aes_basic_byte_leak_count_sens.eps'
#set size 1.2,1.0
#set grid
set title "Cache side-channel leak in AES (basic crypto) w.r.t. cache configurations (observation via miss count)"
set ylabel "No. of impossible values/byte (information leak)" 
set xlabel "Key bytes"
#set xrange [1:10]
set yrange [1:220]
#set logscale y
#set xtics ("2-way, 8KB" 0, "4-way, 8KB" 1, "2-way, 16 KB" 2, "4-way, 16KB" 3, "2-way, 32 KB" 4, "4-way, 32 KB" 5)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3, "5" 4, "6" 5, "7" 6, "8" 7, "9" 8, "10" 9, "11" 10, "12" 11, "13" 12, "14" 13, "15" 14, "16" 15)
#set xtics mirror rotate by 45
#rotate parallel
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
#set style data linespoints

plot 'plots/aes_byte_leak_sensitivity_count.dat' using 1 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 2 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 3 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 4 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 5 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 6 fs pattern 4.66 lt -1 title '4-way, 32 KB'


set title "Cache side-channel leak in AES (OpenSSL) w.r.t. cache configurations (observation via miss count)"
set output 'plots/aes_openssl_byte_leak_count_sens.eps'
set yrange [1:25]

plot 'plots/aes_byte_leak_sensitivity_count.dat' using 13 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 14 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 15 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 16 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 17 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 18 fs pattern 4.66 lt -1 title '4-way, 32 KB'


==> results/scripts/plot_script_test_generation <==
set terminal postscript color
set output 'plots/test_sensitivity.eps'
#set size 1.2,1.0
#set grid
set title "No. of generated tests for varying cache size (LRU)"
set ylabel "#tests"
#set xlabel "cache configurations"
#set xrange [1:10]
set yrange [0:55]
#set logscale y
set xtics ("2-way, 8KB" 0, "4-way, 8KB" 1, "2-way, 16 KB" 2, "4-way, 16KB" 3, "2-way, 32 KB" 4, "4-way, 32 KB" 5, "2-way, 64 KB" 6, "4-way, 64 KB" 7)
set xtics mirror rotate by -45
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
set style data linespoints

plot 'plots/test_generation.dat' using 1 lt -1 lw 2 ps 2 pi -1 pt 6 title 'AES from basic crypto',\
		 '' using 2 lt -1 lw 2 pi -1 pt 7 ps 0.2 title 'AES from OpenSSL',\
		 '' using 3 lt -1 dashtype 3 ps 2 lw 2 pi -1 pt 7 title 'DES',\
		 '' using 4 lt -1 lw 2 ps 2 pi -1 pt 4 title 'RC4',\
		 '' using 5 lt -1 lw 2 ps 2 pi -1 pt 5 title 'GDK'	
		


==> results/scripts/plot_script_test_generation_fifo <==
set terminal postscript color
set output 'plots/test_sensitivity_fifo.eps'
#set size 1.2,1.0
#set grid
set title "No. of generated tests for varying cache size (FIFO)"
set ylabel "#tests"
#set xlabel "cache configurations"
#set xrange [1:10]
set yrange [0:29]
#set logscale y
set xtics ("2-way, 8KB" 0, "4-way, 8KB" 1, "2-way, 16 KB" 2, "4-way, 16KB" 3, "2-way, 32 KB" 4, "4-way, 32 KB" 5, "2-way, 64 KB" 6, "4-way, 64 KB" 7)
set xtics mirror rotate by -45
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
set style data linespoints

plot 'plots/test_generation_fifo.dat' using 1 lt -1 lw 2 ps 2 pi -1 pt 6 title 'AES from basic crypto',\
		 '' using 2 lt -1 lw 2 pi -1 pt 7 ps 0.2 title 'AES from OpenSSL',\
		 '' using 3 lt -1 dashtype 3 ps 2 lw 2 pi -1 pt 7 title 'DES',\
		 '' using 4 lt -1 lw 2 ps 2 pi -1 pt 4 title 'RC4',\
		 '' using 5 lt -1 lw 2 ps 2 pi -1 pt 5title 'GDK'	
		


==> results/scripts/plot_script_test_seq_sens_per_byte <==
set terminal postscript color
set output 'plots/aes_basic_byte_leak_seq_sens.eps'
#set size 1.2,1.0
#set grid
set title "Information leak in AES (basic crypto) w.r.t. cache configurations (observation via hit/miss sequence length 1)"
set ylabel "No. of impossible values/byte (information leak)" 
set xlabel "Key bytes"
#set xrange [1:10]
set yrange [1:256]
#set logscale y
#set xtics ("2-way, 8KB" 0, "4-way, 8KB" 1, "2-way, 16 KB" 2, "4-way, 16KB" 3, "2-way, 32 KB" 4, "4-way, 32 KB" 5)
set xtics ("1" 0, "2" 1, "3" 2, "4" 3, "5" 4, "6" 5, "7" 6, "8" 7, "9" 8, "10" 9, "11" 10, "12" 11, "13" 12, "14" 13, "15" 14, "16" 15)
#set xtics mirror rotate by 45
#rotate parallel
#unset xtics
set boxwidth 0.9 relative
set style histogram
set style data histogram
set style fill solid 1.0 border -1
set border
set key above
#unset key
#set style data linespoints

plot 'plots/aes_byte_leak_sensitivity_seq.dat' using 1 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 2 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 3 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 4 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 5 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 6 fs pattern 4.66 lt -1 title '4-way, 32 KB'


set output 'plots/aes_openssl_byte_leak_seq_sens.eps'
#set yrange [1:]
set title "Information leak in AES (OpenSSL) w.r.t. cache configurations (observation via hit/miss sequence length 1)"

plot 'plots/aes_byte_leak_sensitivity_seq.dat' using 13 fs solid 0.33 lt -1 title '2-way, 8KB',\
		  '' using 14 fs solid 1.33 lt -1 title '4-way, 8KB',\
		  '' using 15 fs pattern 2.00 lt -1 title '2-way, 16KB',\
		  '' using 16 fs pattern 1.33 lt -1 title '4-way, 16KB',\
		  '' using 17 fs pattern 8.66 lt -1 title '2-way, 32 KB',\
		  '' using 18 fs pattern 4.66 lt -1 title '4-way, 32 KB'


==> results/scripts/seq_access_key_bound_script <==
#!/bin/bash

grep -inr "\[++\]" $1 > scripts/leak
while read line; do
	access=$(echo $line | cut -f10 -d" ")
	byte=$(echo $line | cut -f8 -d" ")
	echo $access
	byte=$(echo $byte | rev | cut -c 2- | rev)
	echo $byte
	echo $line >> temp/record_byte_leak_from_hit_sequence_${access}_${byte}
done <scripts/leak
grep -inr "\[--\]" $1 > scripts/leak
while read line; do
	access=$(echo $line | cut -f10 -d" ")
	byte=$(echo $line | cut -f8 -d" ")
	echo $access
	byte=$(echo $byte | rev | cut -c 2- | rev)
	echo $byte
	echo $line >> temp/record_byte_leak_from_miss_sequence_${access}_${byte}
done <scripts/leak



==> results/scripts/splot_script_test <==
# set terminal svg size 600,400 dynamic enhanced fname 'arial'  fsize 10 mousing name "surface1_1" butt dashlength 1.0 
# set output 'surface1.1.svg'
set grid nopolar
set grid xtics nomxtics ytics nomytics noztics nomztics \
 nox2tics nomx2tics noy2tics nomy2tics nocbtics nomcbtics
set grid layerdefault   lt black linewidth 0.200,  lt black linewidth 0.200
set hidden3d back offset 1 trianglepattern 3 undefined 1 altdiagonal bentover
set style data lines
set title "3D surface from a grid (matrix) of Z values" 
set xrange [ -0.500000 : 4.50000 ] noreverse nowriteback
set yrange [ -0.500000 : 4.50000 ] noreverse nowriteback
x = 0.0
splot plots/aes_byte_leak_count.dat with lines notitle


